Using random graphs to sample repulsive Gibbs point processes with arbitrary-range potentials

We study computational aspects of repulsive Gibbs point processes, which are probabilistic models of interacting particles in a finite-volume region of space. We introduce an approach for reducing a Gibbs point process to the hard-core model, a well-studied discrete spin system. Given an instance of such a point process, our reduction generates a random graph drawn from a natural geometric model. We show that the partition function of a hard-core model on graphs generated by the geometric model concentrates around the partition function of the Gibbs point process. Our reduction allows us to use a broad range of algorithms developed for the hard-core model to sample from the Gibbs point process and approximate its partition function. This is, to the extend of our knowledge, the first approach that deals with pair potentials of unbounded range. We compare the resulting algorithms with recently established results and study further properties of the random geometric graphs with respect to the hard-core model.

==> content/discussion.tex <==
\subsection{Discussion and outlook}
We start by having a closer look at the assumptions that we require for our sampling and approximation algorithms to work efficiently.
To this end, let us start by considering the setting where $\region = [0, \ell]^d \subseteq \R^{d}$ is a box of side length $\ell \in \R_{>0}$ in $d$-dimensional Euclidean space, equipped with the Euclidean distance and the Lebesgue measure as volume.  
Our sampling result in \Cref{thm:sampling_simplified} requires an efficient uniform sampler for $\region$.
Note that such a uniform sampler can easily be obtained when assuming a real-valued model of computation, such as given in \cite{blum2000theory}.
The use of such a computational model is not only common \cite{michelen2022strong}, but the ability to output floating point numbers with arbitrary precision is necessary to obtain any non-trivial total variation bound.
In fact, we argue that, even for general complete separable metric spaces, assuming a uniform sampler for a bounded region $\region$ is not a restriction if we aim for sampling from a repulsive Gibbs point processes on $\region$.
To see this, note that any efficient sampler for a Poisson point process with non-zero fugacity (which is a special case of a repulsive Gibbs point process with zero potential) can be turned into an efficient uniform sampler by sampling a non-empty point configuration and selecting one of the points uniformly at random.
Thus, not only does our sampling procedure for repulsive Gibbs point processes require an efficient method for uniform sampling from $\region$, but existence of an efficient sampler for repulsive Gibbs point processes also implies the existence of such a uniform sampler.
For efficient approximation of the partition function, the situation is different.
As shown in \Cref{thm:approximate_gpp}, we only require an efficient sampling procedure for  $\canonicalDistribution{n}{\region}{\potential}$.
This might be possible in some cases without access to a uniform sampler from $\region$.
Especially in the setting of Euclidean space, it could be an interesting question for future research to characterize regions $\region$ and potentials $\potential$ that allow for efficient sampling from $\canonicalDistribution{n}{\region}{\potential}$ with a discrete model of computation.

The next aspect of our results that we discuss is the fugacity regime of $\gppFugacity < \frac{\eulerE}{\generalizedTemperedness{\potential}}$.
In this work, we present the first algorithmic approach that allows for efficient approximation and approximate sampling in that regime for repulsive potentials with infinite range. 
However, in the finite-range setting, \textcite{michelen2022strong} presented a slightly better parameter regime of $\frac{\eulerE}{\connectiveConstant{\potential}}$, where $\connectiveConstant{\potential}$ denotes the potential-weighted connective constant.     
An obvious question is if our approach can achieve the same fugacity bound for general repulsive potentials.
This could be possible by studying the implications that a bound on $\connectiveConstant{\potential}$ has for the random graph model $\canonicalDistribution{n}{\region}{\potential}$, with the goal to achieve better sampling and approximation result for hard-core models on random graphs from that model.
A reasonable candidate for this seems to be the (discrete) connective constant for graphs, which was previously studied in the context of efficient approximation of hard-core partition functions \cite{sinclair2017spatial}.
We believe that further improvements of the fugacity regime and extension to non-repulsive potentials, if possible, will require new conceptual insights.

Our results can be immediately extended to handle Gibbs point processes with non-uniform fugacity.
This is, $\gppFugacity: \pointProcessSpace \to \R_{\ge 0}$ is a measurable function and the Gibbs point process is defined via a density with respect to a Poisson point process of intensity function $\gppFugacity$.
A simple way to model that in the framework of uniform fugacities is to define a new volume measure $\volumeMeasure'(A) = \int_A \gppFugacity(x) \volumeMeasure[\intD x]$ and consider a process of fugacity one with respect to the new reference measure $\volumeMeasure'$.
The resulting process has uniform fugacity and is equivalent to the initial process. Another straightforward extention of our results is to include multiple types of particles. That is, the points are generated from a marked point process and the repulsive potential depents not only on the geometric distance but also on marks of the points.
 
Finally, it would be interesting to see if the concentration inequalities we present in this paper are tight.
As discussed earlier, \Cref{thm:gpp_concentration} is indeed tight in terms of its dependency on $\volumeMeasure[\region]$.
However, to obtain an upper bound on the error probability of $\errorProb \in (0, 1)$, \Cref{thm:gpp_concentration} requires $n \in \bigTheta{\errorProb^{-1}}$.
We wonder if a stronger, Chernoff-like, dependency of $n \in \poly{\ln\left(\errorProb^{-1}\right)}$ can be achieved.
Similarly, it would be interesting if the more general concentration result in \Cref{thm:concentration_partition_function_simplified} is tight, both in terms of the models it applies to and the parameter bound $\fugacity[n] \in \smallO{n^{-\frac{1}{2}}}$.

